A generic characterization of generalized unary temporal logic and two-variable first-order logic

We investigate an operator on classes of languages. For each class $C$, it outputs a new class $FO^2(I_C)$ associated with a variant of two-variable first-order logic equipped with a signature$I_C$ built from $C$. For $C = \{\emptyset, A^*\}$, we get the variant $FO^2(<)$ equipped with the linear order. For $C = \{\emptyset, \{\varepsilon\},A^+, A^*\}$, we get the variant $FO^2(<,+1)$, which also includes the successor. If $C$ consists of all Boolean combinations of languages $A^*aA^*$ where $a$ is a letter, we get the variant $FO^2(<,Bet)$, which also includes "between relations". We prove a generic algebraic characterization of the classes $FO^2(I_C)$. It smoothly and elegantly generalizes the known ones for all aforementioned cases. Moreover, it implies that if $C$ has decidable separation (plus mild properties), then $FO^2(I_C)$ has a decidable membership problem. We actually work with an equivalent definition of \fodc in terms of unary temporal logic. For each class $C$, we consider a variant $TL(C)$ of unary temporal logic whose future/past modalities depend on $C$ and such that $TL(C) = FO^2(I_C)$. Finally, we also characterize $FL(C)$ and $PL(C)$, the pure-future and pure-past restrictions of $TL(C)$. These characterizations as well imply that if \Cs is a class with decidable separation, then $FL(C)$ and $PL(C)$ have decidable membership.

==> macros.tex <==
\usepackage{xspace}
\usepackage{bbm}
\usepackage{thmtools,thm-restate}
\usepackage{csquotes}
\usepackage{nowidow}
\usepackage{widows-and-orphans}
 % \usepackage[All]{lua-typo}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing,hobby,backgrounds,trees,arrows,automata,shapes,positioning,fit,patterns,calc,matrix}

%%%%%%% Basic stuff %%%%%%

\newcommand{\veps}{\ensuremath{\varepsilon}\xspace}
%\newcommand{\uclos}{\ensuremath{\mathord{\uparrow}}\xspace}
\newcommand{\inv}{^{-1}}
\newcommand{\nat}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\integ}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\frB}{\ensuremath{\mathbb{B}}\xspace}
\newcommand{\frP}{\ensuremath{\mathbb{P}}\xspace}
\newcommand{\fri}{\ensuremath{\mathbbm{i}}\xspace}
\newcommand{\frS}{\ensuremath{\mathbbm{S}}\xspace}
\newcommand{\cont}[1]{\ensuremath{\mathit{alph}(#1)}\xspace}

%%%%%% Fonts %%%%%%

\newcommand{\As}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\Bs}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\Cs}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\Ds}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\Es}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\Fs}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\Gs}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\Hs}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\Is}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\Js}{\ensuremath{\mathcal{J}}\xspace}
\newcommand{\Ks}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\Ls}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Ms}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\Ns}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\Os}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\Ps}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Qs}{\ensuremath{\mathcal{Q}}\xspace}
\newcommand{\Rs}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\Ss}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\Ts}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\Us}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\Vs}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\Ws}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\Xs}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\Ys}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\Zs}{\ensuremath{\mathcal{Z}}\xspace}

\newcommand{\Ab}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\Bb}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\Cb}{\ensuremath{\mathbf{C}}\xspace}
\newcommand{\Db}{\ensuremath{\mathbf{D}}\xspace}
\newcommand{\Eb}{\ensuremath{\mathbf{E}}\xspace}
\newcommand{\Fb}{\ensuremath{\mathbf{F}}\xspace}
\newcommand{\Gb}{\ensuremath{\mathbf{G}}\xspace}
\newcommand{\Hb}{\ensuremath{\mathbf{H}}\xspace}
\newcommand{\Ib}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\Jb}{\ensuremath{\mathbf{J}}\xspace}
\newcommand{\Kb}{\ensuremath{\mathbf{K}}\xspace}
\newcommand{\Lb}{\ensuremath{\mathbf{L}}\xspace}
\newcommand{\Mb}{\ensuremath{\mathbf{M}}\xspace}
\newcommand{\Nb}{\ensuremath{\mathbf{N}}\xspace}
\newcommand{\Ob}{\ensuremath{\mathbf{O}}\xspace}
\newcommand{\Pb}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\Qb}{\ensuremath{\mathbf{Q}}\xspace}
\newcommand{\Rb}{\ensuremath{\mathbf{R}}\xspace}
\newcommand{\Sb}{\ensuremath{\mathbf{S}}\xspace}
\newcommand{\Tb}{\ensuremath{\mathbf{T}}\xspace}
\newcommand{\Ub}{\ensuremath{\mathbf{U}}\xspace}
\newcommand{\Vb}{\ensuremath{\mathbf{V}}\xspace}
\newcommand{\Wb}{\ensuremath{\mathbf{W}}\xspace}
\newcommand{\Xb}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\Yb}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\Zb}{\ensuremath{\mathbf{Z}}\xspace}

%%%%%%%%%%%%% Varieties and Stuff %%%%%%%%%%%%

\newcommand{\wsuit}{well-suited\xspace}
\newcommand{\Wsuit}{Well-suited\xspace}

\newcommand{\vari}{prevariety\xspace}
\newcommand{\Vari}{Prevariety\xspace}
\newcommand{\varis}{prevarieties\xspace}
\newcommand{\Varis}{Prevarieties\xspace}

\newcommand{\pvari}{positive prevariety\xspace}
\newcommand{\pVari}{Positive prevariety\xspace}
\newcommand{\pvaris}{positive prevarieties\xspace}
\newcommand{\pVaris}{Positive prevarieties\xspace}

\newcommand{\prefsig}[1]{\ensuremath{\mathbb{P}_{#1}}\xspace}
\newcommand{\infsig}[1]{\ensuremath{\mathbb{I}_{#1}}\xspace}
\newcommand{\infsigc}{\infsig{\Cs}}



%%%%%% Complex %%%%%

% Time

\newcommand{\ptime}{\textup{\sc P}\xspace}
\newcommand{\nptime}{\textup{\sc NP}\xspace}
\newcommand{\conptime}{\textup{co-{\sc NP}}\xspace}
\newcommand{\poracle}{\ensuremath{{\text{\sc P}}^{{\text{\sc NP}}}}\xspace}
\newcommand{\exptime}{\textup{\sc EXPTIME}\xspace}
\newcommand{\pexptime}[1]{\textup{#1-}{\sc EXPTIME}\xspace}
\newcommand{\nexptime}{\textup{\sc NEXPTIME}\xspace}
\newcommand{\conexptime}{\textup{co-{\sc NEXPTIME}}\xspace}
\newcommand{\pnexptime}[1]{\textup{#1-}{\sc NEXPTIME}\xspace}
\newcommand{\exporacle}{\ensuremath{{\text{\sc EXPTIME}}^{{\text{\sc NEXPTIME}}}}\xspace}
\newcommand{\pexporacle}[1]{\ensuremath{{\textup{#1-}\text{\sc EXPTIME}}^{\textup{#1-}{\text{\sc NEXPTIME}}}}\xspace}
% Space

\newcommand{\logspace}{\textup{\sc LOGSPACE}\xspace}
\newcommand{\nl}{\textup{{\sc NL}}\xspace}
\newcommand{\conl}{\textup{co-{\sc NL}}\xspace}
\newcommand{\pspace}{\textup{\sc PSPACE}\xspace}
\newcommand{\npspace}{\textup{\sc NPSPACE}\xspace}
\newcommand{\expspace}{\textup{\sc EXPSPACE}\xspace}
\newcommand{\pexpspace}[1]{\textup{#1-}{\sc EXPSPACE}\xspace}


%%%%% Automata %%%%%%

\newcommand{\nfa}{{{NFA}}\xspace}
\newcommand{\pnfa}{pre-NFA\xspace}
\newcommand{\dfa}{{{DFA}}\xspace}

\newcommand{\nfas}{{\textup{NFAs}}\xspace}
\newcommand{\pnfas}{{\textup{pre-NFAs}}\xspace}
\newcommand{\dfas}{{\textup{DFAs}}\xspace}

\newcommand{\nfaps}{{\textup{NFA(s)}}\xspace}
\newcommand{\pnfaps}{{\textup{pre-NFA(s)}}\xspace}
\newcommand{\dfaps}{{\textup{DFA(s)}}\xspace}

\newcommand{\lauto}[3]{\ensuremath{L_{#1}(#2,#3)}\xspace}
\newcommand{\alauto}[2]{\lauto{\As}{#1}{#2}}


%%%%%%%% Ratms %%%%%%

\newcommand{\dnsep}[2]{\ensuremath{\Is_{#1}[\Ds,#2]}\xspace}
\newcommand{\dnsepca}{\dnsep{\Cs}{\As}}
\newcommand{\gnsep}[2]{\ensuremath{\Is_{#1}[\Gs,#2]}\xspace}
\newcommand{\gnsepca}{\gnsep{\Cs}{\As}}
\newcommand{\gnsepda}{\gnsep{\Ds}{\As}}
\newcommand{\gnsepbpa}{\gnsep{\bpol{\Ds}}{\As}}

\newcommand{\dclos}{\ensuremath{\mathord{\downarrow}}\xspace}
\newcommand{\uclos}{\ensuremath{\mathord{\uparrow}}\xspace}

\newcommand{\dclosp}[1]{\ensuremath{\mathord{\downarrow_{#1}}}\xspace}
\newcommand{\dclosr}{\dclosp{R}}
\newcommand{\dclosq}{\dclosp{Q}}

%%%%%%%%%%%%%%%% Vocabulary %%%%%%%%%%%%%%%%
\newcommand{\imprint}{imprint\xspace}
\newcommand{\imprints}{imprints\xspace}
\newcommand{\Imprint}{Imprint\xspace}
\newcommand{\Imprints}{Imprints\xspace}

\newcommand{\iden}{\veps-approximation\xspace}
\newcommand{\idens}{\veps-approximations\xspace}
\newcommand{\Iden}{\veps-Approximation\xspace}
\newcommand{\Idens}{\veps-Approximations\xspace}

%\newcommand{\ope}{\ensuremath{\odot}\xspace}

\newcommand{\tame}{multiplicative\xspace}
\newcommand{\Tame}{Multiplicative\xspace}
\newcommand{\wtame}{weak multiplicative\xspace}

\newcommand{\Ratms}{Rating maps\xspace}
\newcommand{\Ratm}{Rating map\xspace}
\newcommand{\ratms}{rating maps\xspace}
\newcommand{\ratm}{rating map\xspace}
\newcommand{\Rata}{Rating algebra\xspace}
\newcommand{\Ratas}{Rating algebras\xspace}
\newcommand{\rata}{rating algebra\xspace}
\newcommand{\ratas}{rating algebras\xspace}


\newcommand{\Nice}{Nice\xspace}
\newcommand{\nice}{nice\xspace}
\newcommand{\effective}{effective\xspace}

\newcommand{\mratm}{multiplicative rating map\xspace}
\newcommand{\mratms}{multiplicative rating maps\xspace}
\newcommand{\Mratm}{Multiplicative rating map\xspace}
\newcommand{\Mratms}{Multiplicative rating maps\xspace}

\newcommand{\pratm}{powerset rating map\xspace}
\newcommand{\pratms}{powerset rating map\xspace}
\newcommand{\Pratm}{Powerset rating map\xspace}
\newcommand{\Pratms}{Powerset rating map\xspace}


\newcommand{\wmratm}{weak multiplicative rating map\xspace}
\newcommand{\wmratms}{weak multiplicative rating maps\xspace}
\newcommand{\Wmratm}{Weak multiplicative rating map\xspace}
\newcommand{\Wmratms}{Weak multiplicative rating maps\xspace}

\newcommand{\gfil}[2]{\ensuremath{\tau^{#2}_{#1}}\xspace}
\newcommand{\gfiln}{\gfil{\Lb,\Ds}{n}}
\newcommand{\gfilp}{\gfil{\Lb}{n}\xspace}
\newcommand{\gfilpp}[1]{\gfil{\Lb}{#1}\xspace}

\newcommand{\fixg}[3]{\ensuremath{Red_{#1}^{#2}(#3)}\xspace}
\newcommand{\fixgln}[1]{\fixg{\alpha}{n}{#1}}


\newcommand{\sdrat}{\ensuremath{\zeta_{\alpha,\rho}}\xspace}
\newcommand{\drat}[1]{\ensuremath{\zeta^{#1}_{\alpha,\rho}}\xspace}
\newcommand{\dratp}[2]{\ensuremath{\zeta^{#1}_{#2}}\xspace}

\newcommand{\sgrat}{\ensuremath{\xi_{\rho}}\xspace}
\newcommand{\grat}[1]{\ensuremath{\xi^{#1}_{\rho}}\xspace}

\newcommand{\quasi}[1]{\ensuremath{\mu_{#1}}\xspace}
\newcommand{\quasir}{\quasi{\rho}}
\newcommand{\quasit}{\quasi{\tau}}
\newcommand{\quasig}{\quasi{\gamma}}

\newcommand{\brataux}[2]{\ensuremath{\xi_{#1}[#2]}\xspace}
\newcommand{\bratauxc}{\brataux{\Cs}{\rho}}
\newcommand{\bratauxd}{\brataux{\Ds}{\rho}}
\newcommand{\bratauxbd}{\brataux{\bool{\Ds}}{\rho}}
\newcommand{\bratauxbc}{\brataux{\bpol{\Cs}}{\rho}}
\newcommand{\bratauxsfc}{\brataux{\sfp{\Cs}}{\rho}}

\newcommand{\bratauxbg}{\brataux{\bpol{\Gs}}{\rho}}
\newcommand{\bratauxsfg}{\brataux{\sfp{\Gs}}{\rho}}

\newcommand{\bratauxbw}{\brataux{\bpol{\Gs^+}}{\rho}}


\newcommand{\lrataux}[3]{\ensuremath{\zeta_{#1}[#2,#3]}\xspace}
\newcommand{\lratauxc}{\lrataux{\Cs}{\alpha}{\rho}}
\newcommand{\lratauxd}{\lrataux{\Ds}{\alpha}{\rho}}
\newcommand{\lratauxpc}{\lrataux{\pol{\Cs}}{\alpha}{\rho}}
\newcommand{\lratauxppc}{\lrataux{\pbpol{\Cs}}{\alpha}{\rho}}
\newcommand{\lratauxpnc}{\lrataux{\pbpol{\Cs}}{\nu}{\rho}}
\newcommand{\lratauxpd}{\lrataux{\pol{\Ds}}{\nu}{\rho}}

\newcommand{\lratrp}[2]{\lrataux{#1}{#2}{\rho}}
\newcommand{\lratdrp}[1]{\lrataux{\Ds}{#1}{\rho}}
\newcommand{\lratdrn}{\lratdrp{n}}

\newcommand{\lratauxpng}{\lrataux{\pbpol{\Gs}}{\nu}{\rho}}

\newcommand{\lratauxpg}{\lrataux{\pol{\Gs}}{\alpha}{\rho}}
\newcommand{\lratauxppg}{\lrataux{\pbpol{\Gs}}{\alpha}{\rho}}

\newcommand{\lratauxppw}{\lrataux{\pbpol{\Gs^+}}{\alpha}{\rho}}

%%%%%%%%%%%%%%%% Notations Imprints %%%%%%%%%%%%%%%%%


\newcommand{\prin}[2]{\ensuremath{\Is[#1](#2)}\xspace}

\newcommand{\itriv}[1]{\ensuremath{\Is_{\mathit{triv}}[#1]}\xspace}
\newcommand{\ptriv}[1]{\ensuremath{\Ps_{\mathit{triv}}[#1]}\xspace}

\newcommand{\opti}[2]{\ensuremath{\Is_{#1}\left[#2\right]}\xspace}
\newcommand{\copti}[1]{\opti{\Cs}{#1}}
\newcommand{\dopti}[1]{\opti{\Ds}{#1}}
\newcommand{\gopti}[1]{\opti{\Gs}{#1}}
\newcommand{\popti}[3]{\ensuremath{\Ps_{#1}[#2,#3]}\xspace}
\newcommand{\pcopti}[2]{\popti{\Cs}{#1}{#2}}
\newcommand{\pdopti}[2]{\popti{\Ds}{#1}{#2}}

\newcommand{\iopti}[2]{\ensuremath{\fri_{#1}[#2]}\xspace}
\newcommand{\ioptic}[1]{\iopti{\Cs}{#1}}
\newcommand{\ioptid}[1]{\iopti{\Ds}{#1}}
\newcommand{\ioptig}[1]{\iopti{\Gs}{#1}}


\newcommand{\nsep}[2]{\ensuremath{\Is_{#1}[#2]}\xspace}
\newcommand{\nsepc}[1]{\nsep{\Cs}{#1}}
\newcommand{\nsepcm}{\nsepc{\alpha}}
\newcommand{\nsepca}{\nsepc{\As}}
\newcommand{\nsepd}[1]{\nsep{\Ds}{#1}}
\newcommand{\nsepdm}{\nsepd{\alpha}}
\newcommand{\nsepda}{\nsepd{\As}}

\newcommand{\nsepbca}{\nsep{\bpol{\Cs}}{\As}}
\newcommand{\gnsepbca}{\nsep{\bpol{\Cs}}{\Gs,\As}}

%%%%%%% Imprint reduction for BPol  %%%%%%%%%%%

% Generic carac
\newcommand{\rbpol}[1]{\ensuremath{\Rs^\rho_{#1}}\xspace}
\newcommand{\rbpols}{\ensuremath{\rbpol{S}}\xspace}
\newcommand{\rbpolt}{\ensuremath{\rbpol{T}}\xspace}

\newcommand{\tbpol}[1]{\ensuremath{\Rs_\tau(#1)}\xspace}
\newcommand{\tbpols}{\ensuremath{\tbpol{S}}\xspace}

% ST1 carac
\newcommand{\redstone}[1]{\ensuremath{\Ss\Ts^{1,\rho}_{#1}}\xspace}
\newcommand{\redstones}{\redstone{S}}

% DD1 carac
\newcommand{\reddotone}[1]{\ensuremath{\Ds\Ds^{1,\rho}_{#1}}\xspace}
\newcommand{\reddotones}{\reddotone{S}}

% ST2 carac
\newcommand{\rstd}[1]{\ensuremath{\Ss\Ts^{2,\rho}_{#1}}\xspace}
\newcommand{\rstds}{\rstd{S}}

%%%% Tied tuples


\newcommand{\ttup}[3]{\ensuremath{\Ts_{#1}^{#2}[{#3}]}\xspace}
\newcommand{\polttup}[1]{\ttup{\pol{\Cs}}{#1}{\Lb}}
\newcommand{\polttupn}{\polttup{n}}

\newcommand{\stup}[1]{\ensuremath{\Ts^{#1}[\Lb]}\xspace}
\newcommand{\stupn}{\stup{n}}
\newcommand{\stupnm}{\stup{n-1}}

\newcommand{\alte}[3]{\ensuremath{\As_{#1}^{#2}[#3]}\xspace}
\newcommand{\polalte}[1]{\alte{\pol{\Cs}}{#1}{\Lb}}


\newcommand{\salte}{\ensuremath{\As[\Lb]}\xspace}

\newcommand{\ite}[2]{\ensuremath{it_{#1}(#2)}\xspace}
\newcommand{\iteh}[1]{\ite{h}{#1}}

\newcommand{\extra}[2]{\ensuremath{ex_{#1}(#2)}\xspace}


\newcommand{\gfix}[1]{\ensuremath{Res(#1)}\xspace}

%%% Groups
\newcommand{\igrpopti}{\iopti{\grp}{\rho}}
\newcommand{\grpopti}{\opti{\grp}{\rho}}
\newcommand{\mdopti}{\opti{\md}{\rho}}


%%%% LT-LTT
\newcommand{\atopti}{\opti{\at}{\rho}}
\newcommand{\attopti}{\opti{\att}{\rho}}
\newcommand{\ltopti}{\opti{\lt}{\rho}}
\newcommand{\lttopti}{\opti{\ltt}{\rho}}

%%%% BSigma1

\newcommand{\bsuopti}{\opti{\bscu}{\rho}}
\newcommand{\ptopti}{\opti{\pt}{\rho}}
\newcommand{\pptopti}{\popti{\ppt}{\alpha}{\rho}}

%%%% FO2

\newcommand{\fodopti}{\opti{\ul}{\rho}}
\newcommand{\fodpopti}{\popti{\ul}{\etaat}{\rho}}

%%%% FO SF

\newcommand{\foopti}{\opti{\fo}{\rho}}
\newcommand{\sfopti}{\opti{\sfr}{\rho}}

\newcommand{\sfsatag}{\sata{G}{\rho}}
\newcommand{\sfsatah}{\sata{H}{\rho}}

%%%% PolC

\newcommand{\powgopti}{\popti{\pol{\Gs^+}}{\alpha}{\rho}}
\newcommand{\bpwgopti}{\opti{\bpol{\Gs^+}}{\rho}}
\newcommand{\pbpwgopti}{\popti{\pbpol{\Gs^+}}{\alpha}{\rho}}

\newcommand{\pogopti}{\popti{\pol{\Gs}}{\alpha}{\rho}}
\newcommand{\bpgopti}{\opti{\bpol{\Gs}}{\rho}}
\newcommand{\pbpgopti}{\popti{\pbpol{\Gs}}{\alpha}{\rho}}

\newcommand{\pocopti}{\popti{\pol{\Cs}}{\alpha}{\rho}}
\newcommand{\cpocopti}{\popti{\pol{\Cs}}{\etac,\alpha}{\rho}}
\newcommand{\bpopti}{\opti{\bpol{\Cs}}{\rho}}
\newcommand{\cbpopti}{\popti{\bpol{\Cs}}{\etac}{\rho}}
\newcommand{\pbpopti}{\popti{\pbpol{\Cs}}{\alpha}{\rho}}
\newcommand{\cpbpopti}{\popti{\pbpol{\Cs}}{\etac,\alpha}{\rho}}
\newcommand{\sfcopti}{\opti{\sfp{\Cs}}{\rho}}
\newcommand{\csfcopti}{\popti{\sfp{\Cs}}{\etac}{\rho}}

\newcommand{\stau}{\ensuremath{\overline{\tau}}\xspace}
\newcommand{\sgamma}{\ensuremath{\overline{\gamma}}\xspace}
%\newcommand{\tpocopti}{\popti{\pol{\Cs}}{\etac,\rho_*}{\tau}}
\newcommand{\gpocopti}{\popti{\pol{\Cs}}{\etac,\rho_*}{\gamma}}

\newcommand{\sthoneopti}{\popti{\sthone}{\alpha}{\rho}}
\newcommand{\sthtwoopti}{\popti{\sthtwo}{\alpha}{\rho}}
\newcommand{\asthtwoopti}{\popti{\sthtwo}{\etaat,\alpha}{\rho}}
\newcommand{\sththropti}{\popti{\sththree}{\alpha}{\rho}}
\newcommand{\asththropti}{\popti{\sththree}{\etaat,\alpha}{\rho}}

\newcommand{\stoneopti}{\opti{\stone}{\rho}}
\newcommand{\dotoneopti}{\opti{\dotone}{\rho}}
\newcommand{\sttwoopti}{\opti{\sttwo}{\rho}}
\newcommand{\asttwoopti}{\popti{\sttwo}{\etaat}{\rho}}
\newcommand{\dothoneopti}{\popti{\dothone}{\alpha}{\rho}}
\newcommand{\dothtwoopti}{\popti{\dothtwo}{\alpha}{\rho}}

\newcommand{\upolopti}{\opti{\upol{\Cs}}{\rho}}
\newcommand{\ldetopti}{\opti{\ldet{\Cs}}{\rho}}
\newcommand{\rdetopti}{\opti{\rdet{\Cs}}{\rho}}
\newcommand{\ldetnopti}{\opti{\ldetn{\Cs}}{\rho}}
\newcommand{\rdetnopti}{\opti{\rdetn{\Cs}}{\rho}}

\newcommand{\pupolopti}{\popti{\upol{\Cs}}{\etac}{\rho}}
\newcommand{\pldetopti}{\popti{\ldet{\Cs}}{\etac}{\rho}}
\newcommand{\pldetoptid}{\popti{\ldet{\Ds}}{\etac}{\rho}}
\newcommand{\prdetopti}{\popti{\rdet{\Cs}}{\etac}{\rho}}
\newcommand{\prdetoptid}{\popti{\rdet{\Ds}}{\etac}{\rho}}
\newcommand{\pmdetopti}{\popti{\mdet{\Cs}}{\etac}{\rho}}
\newcommand{\pmdetoptid}{\popti{\mdet{\Ds}}{\etac}{\rho}}
\newcommand{\pldetnopti}{\popti{\ldetn{\Cs}}{\etac}{\rho}}
\newcommand{\pldetnmopti}{\popti{\ldetp{n-1}{\Cs}}{\etac}{\rho}}
\newcommand{\prdetnopti}{\popti{\rdetn{\Cs}}{\etac}{\rho}}
\newcommand{\prdetnmopti}{\popti{\rdetp{n-1}{\Cs}}{\etac}{\rho}}
\newcommand{\pmdetnopti}{\popti{\mdetn{\Cs}}{\etac}{\rho}}
\newcommand{\pmdetnmopti}{\popti{\mdetp{n-1}{\Cs}}{\etac}{\rho}}

%%%% Compatibility

\newcommand{\typ}[2]{\ensuremath{[#1]_{#2}}\xspace}
\newcommand{\ctype}[1]{\typ{#1}{\Cs}}
\newcommand{\pctype}[1]{\typ{#1}{\pol{\Cs}}}
\newcommand{\cmult}{\ensuremath{\mathbin{\scriptscriptstyle\bullet}}}
\newcommand{\dtype}[1]{\typ{#1}{\Ds}}
\newcommand{\gtype}[1]{\typ{#1}{\Gs}}


\newcommand{\rtyp}[2]{\ensuremath{\llbracket #1 \rrbracket_{#2}}\xspace}
\newcommand{\crtype}[1]{\rtyp{#1}{\Cs}}
\newcommand{\ertype}[1]{\rtyp{#1}{\varepsilon}}

\newcommand{\sztyp}[1]{\typ{#1}{\stzer}}
\newcommand{\szrtyp}[1]{\rtyp{#1}{\stzer}}

\newcommand{\dztyp}[1]{\typ{#1}{\dotzer}}
\newcommand{\dzrtyp}[1]{\rtyp{#1}{\dotzer}}

\newcommand{\compset}[2]{\ensuremath{\fil{\alpha}{\typ{#2}{#1}}}\xspace}
\newcommand{\compsetc}[1]{\compset{\Cs}{#1}}


%%%% Auxiliary ratms

\newcommand{\alrat}{\ensuremath{\nu^{\alpha}_{\rho}}\xspace}
\newcommand{\abrat}{\ensuremath{\nu_{\rho}}\xspace}

\newcommand{\glrat}[1]{\ensuremath{\nu^{\alpha}_{\rho,#1}}\xspace}
\newcommand{\glrats}{\glrat{S}}

% BPolG
\newcommand{\bwmrat}[1]{\ensuremath{\eta_{\rho,#1}}\xspace}
\newcommand{\bwmrats}{\bwmrat{S}}

% BPolG+
\newcommand{\bpwmrat}[1]{\ensuremath{\lambda_{\rho,#1}}\xspace}
\newcommand{\bpwmrats}{\bpwmrat{S}}
\newcommand{\idpr}{\ensuremath{E_+(\rho)}\xspace}

% PBPolG
\newcommand{\pbwmrat}[1]{\ensuremath{\delta^{\alpha}_{\rho,#1}}\xspace}
\newcommand{\pbwmrats}{\pbwmrat{S}}

%PBPolG+
\newcommand{\pwbwmrat}[1]{\ensuremath{\mu^{\alpha}_{\rho,#1}}\xspace}
\newcommand{\pwbwmrats}{\pwbwmrat{S}}
\newcommand{\idpar}{\ensuremath{E_+(\alpha,\rho)}\xspace}







%%%%%%%%%%% Automata %%%%%%%%%%%%%%%%
\usepackage{tikz}
\usetikzlibrary{automata}

\tikzset{every state/.style={draw=blue!50!green,very thick,fill=blue!50!green!20}}
\tikzset{statesub/.style={state,minimum size=1.3cm,inner sep=1pt}}
\tikzset{pattstate/.style={state,draw=red!50!yellow,line width=2pt,fill=red!50!yellow!20}}
\tikzset{pdotstate/.style={state,minimum size=0.75cm,inner sep=0.5pt,draw=red!50!yellow,line
		width=2pt,dashed,fill=red!50!yellow!20}}
\tikzset{lstate/.style={state,minimum size=0.65cm,inner sep=0.5pt}}
\tikzstyle{trans}=[shorten >= 1pt,thick,->]

\makeatletter
\tikzstyle{initial by arrow}=   [after node path=
{
	{
		[to path=
		{
			[->,double=none,shorten >= 1pt,thick,every initial by arrow]
			([shift=(\tikz@initial@angle:\tikz@initial@distance)]\tikztostart.\tikz@initial@angle)
			node [shape=coordinate,anchor=\tikz@initial@anchor,draw] {\tikz@initial@text}
			-- (\tikztostart)}]
		edge ()
	}
}]
\makeatother

\makeatletter
\tikzstyle{accepting by arrow}=   [after node path=
{
	{
		[to path=
		{
			[->,double=none,shorten >= 1pt,thick,every accepting by arrow]
			(\tikztostart) -- 
			([shift=(\tikz@accepting@angle:\tikz@accepting@distance)]\tikztostart.\tikz@accepting@angle)
			node [shape=coordinate,anchor=\tikz@accepting@anchor,draw] {\tikz@accepting@text}
		}
		]
		edge ()
	}
}]
\makeatother

% \mvline[<style>]{<matrix name>}{<column number on the right hand side of the line>}
\newcommand{\mvline}[3][]{%
	\pgfmathtruncatemacro\hc{#3-1}
	\draw[#1]({$(#2-1-#3.west)!.5!(#2-1-\hc.east)$} |- #2.north) -- ({$(#2-1-#3.west)!.5!(#2-1-\hc.east)$} |- #2.south);
}
% \mhline[<style>]{<matrix name>}{<row number below of the line>}{<number of columns in a row>}
\newcommand{\mhline}[3][]{%
	\pgfmathtruncatemacro\hc{#3-1}
	\node[fit=(#2-#3-1),inner sep=0pt](R){};
	\node[fit=(#2-\hc-1),inner sep=0pt](L){};
	\node (K) at ($(R)!0.5!(L)$) {};
	\draw[#1] (K -| #2.west) -- (K -| #2.east);
}

\newcommand{\mhlinel}[3][]{%
	\pgfmathtruncatemacro\hc{#3-1}
	\node[fit=(#2-#3-2),inner sep=0pt](R){};
	\node[fit=(#2-\hc-2),inner sep=0pt](L){};
	\node (K) at ($(R)!0.5!(L)$) {};
	\draw[#1] (K -| #2.west) -- (K -| #2.east);
}

%%%%% Startification generic %%%%%

\newcommand{\pstr}[2]{\ensuremath{#1\textup{-}{#2}}\xspace}
\newcommand{\pstc}[1]{\pstr{#1}{\Cs}}
\newcommand{\kstc}{\pstc{k}}


%%%%%% Concatenation hierarchy generic %%%%%

\newcommand{\hiep}[2]{\ensuremath{#1_{#2}}\xspace}
\newcommand{\hiec}[1]{\hiep{\Cs}{#1}}
\newcommand{\hied}[1]{\hiep{\Ds}{#1}}
\newcommand{\hieg}[1]{\hiep{\Gs}{#1}}


\newcommand{\hiesp}[2]{\ensuremath{(#1^+)_{#2}}\xspace}
\newcommand{\hiesc}[1]{\hiesp{\Cs}{#1}}
\newcommand{\hiesg}[1]{\hiesp{\Gs}{#1}}


%%%%% Predicates %%%%%
\let\omin\min
\let\omax\max
\renewcommand{\min}{\ensuremath{\text{\scriptsize min}}\xspace}
\renewcommand{\max}{\ensuremath{\text{\scriptsize max}}\xspace}


\newcommand{\mods}{\ensuremath{\mathit{MOD}}\xspace}
\newcommand{\amods}{\ensuremath{\mathit{AMOD}}\xspace}

\newcommand{\amodp}[3]{\ensuremath{\mathit{MOD}^{#1}_{#2,#3}}\xspace}
\newcommand{\amodamd}{\amodp{a}{m}{d}}

\newcommand{\modp}[2]{\ensuremath{\mathit{MOD}_{#1,#2}}\xspace}
\newcommand{\modmd}{\modp{m}{d}}

\newcommand{\sigenr}{\ensuremath{<,+1,\min,\max,\varepsilon}\xspace}
\newcommand{\addsucc}{\ensuremath{+1,\min,\max,\varepsilon}\xspace}

%%%%%%% Convention %%%%%%%%%%
%w  = order
%ws = enriched
%p  = successor
%eq = equality

%%%%% The Two Main Ones %%%%%
\newcommand{\fo}{\ensuremath{\textup{FO}}\xspace}
\newcommand{\fow}{\mbox{\ensuremath{\fo(<)}}\xspace}
\newcommand{\fows}{\mbox{\ensuremath{\fo(<,+1)}}\xspace}
\newcommand{\fowss}{\mbox{\ensuremath{\fo(\sigenr)}}\xspace}
\newcommand{\foeqp}{\mbox{\ensuremath{\fo(+1)}}\xspace}
%\newcommand{\fopm}{\mbox{\ensuremath{\fo(+1,\min,\max)}}\xspace}
\newcommand{\foeq}{\mbox{\ensuremath{\fo(\emptyset)}}\xspace}
\newcommand{\fop}{\mbox{\ensuremath{\fo(+1)}}\xspace}
\newcommand{\foc}{\ensuremath{\fo(\infsigc)}\xspace}

\newcommand{\fowam}{\mbox{\ensuremath{\fo(<,\amods)}}\xspace}
\newcommand{\fowsam}{\mbox{\ensuremath{\fo(<,+1,\amods)}}\xspace}



\newcommand{\fowm}{\mbox{\ensuremath{\fo(<,\mods)}}\xspace}
\newcommand{\fowsm}{\mbox{\ensuremath{\fo(<,+1,\mods)}}\xspace}
\newcommand{\foeqpm}{\mbox{\ensuremath{\fo(=,+1,\mods)}}\xspace}
\newcommand{\fopm}{\mbox{\ensuremath{\fo(+1,\mods)}}\xspace}
\newcommand{\foeqm}{\mbox{\ensuremath{\fo(=,\mods)}}\xspace}


\newcommand{\rec}{\ensuremath{\textup{REC}}\xspace}
\newcommand{\reg}{\ensuremath{\textup{REG}}\xspace}
\newcommand{\mso}{\ensuremath{\textup{MSO}}\xspace}
\newcommand{\msow}{\ensuremath{\mso(<)}\xspace}
\newcommand{\msows}{\ensuremath{\mso(<,+1,\mods)}\xspace}
\newcommand{\msowsa}{\ensuremath{\mso(<,+1,\amods)}\xspace}
\newcommand{\msop}{\ensuremath{\mso(+1)}\xspace}
\newcommand{\msono}{\mso without first-order variables\xspace}

%%%%% Variables Restrictions %%%%%
\newcommand{\fou}{\ensuremath{\fo^1}\xspace}
\newcommand{\fod}{\ensuremath{\fo^2}\xspace}
\newcommand{\fot}{\ensuremath{\fo^3}\xspace}
\newcommand{\foi}{\ensuremath{\fo^i}\xspace}
\newcommand{\fodc}{\ensuremath{\fod(\infsigc)}\xspace}


\newcommand{\folab}{\mbox{\ensuremath{\fou(\emptyset)}}\xspace}
\newcommand{\folabm}{\mbox{\ensuremath{\fou(\mods)}}\xspace}
\newcommand{\folabam}{\mbox{\ensuremath{\fou(\amods)}}\xspace}
\newcommand{\fouw}{\ensuremath{\fou(<)}\xspace}
\newcommand{\foueq}{\ensuremath{\fou(=)}\xspace}
\newcommand{\foup}{\ensuremath{\fou(+1)}\xspace}


\newcommand{\fodw}{\ensuremath{\fod(<)}\xspace}
\newcommand{\fodws}{\ensuremath{\fod(<,+1)}\xspace}
\newcommand{\fodeq}{\ensuremath{\fod(=)}\xspace}
\newcommand{\fodp}{\ensuremath{\fod(+1)}\xspace}
\newcommand{\fodwm}{\ensuremath{\fod(<,\mods)}\xspace}
\newcommand{\fodwam}{\ensuremath{\fod(<,\amods)}\xspace}
\newcommand{\fodwsm}{\ensuremath{\fod(<,+1,\mods)}\xspace}
\newcommand{\fodwsam}{\ensuremath{\fod(<,+1,\amods)}\xspace}
\newcommand{\fodreg}{\ensuremath{\fod(REG)}\xspace}


\newcommand{\fodsi}[1]{\ensuremath{\sic{#1}^2}\xspace}
\newcommand{\fodsn}{\fodsi{n}}

\newcommand{\fodpi}[1]{\ensuremath{\pic{#1}^2}\xspace}
\newcommand{\fodpn}{\fodpi{n}}

\newcommand{\fodb}[1]{\ensuremath{\bsc{#1}^2}\xspace}
\newcommand{\fodbn}{\fodb{n}}


\newcommand{\foieq}{\ensuremath{\foi(=)}\xspace}
\newcommand{\foip}{\ensuremath{\foi(+1)}\xspace}

\newcommand{\fotw}{\ensuremath{\fot(<)}\xspace}
\newcommand{\foiw}{\ensuremath{\foi(<)}\xspace}



\newcommand{\fodiw}{\ensuremath{\fo^2_i(<)}\xspace}
\newcommand{\foduw}{\ensuremath{\fo^2_1(<)}\xspace}
\newcommand{\foddw}{\ensuremath{\fo^2_2(<)}\xspace}
\newcommand{\fodtw}{\ensuremath{\fo^2_3(<)}\xspace}

\newcommand{\fodiws}{\ensuremath{\fo^2_i(<,+1)}\xspace}
\newcommand{\foduws}{\ensuremath{\fo^2_1(<,+1,\min,\max)}\xspace}
\newcommand{\foddws}{\ensuremath{\fo^2_2(<,+1)}\xspace}
\newcommand{\fodtws}{\ensuremath{\fo^2_3(<,+1)}\xspace}


%%%%% Quantifier Alternation FO %%%%%

% Sigma
\newcommand{\sic}[1]{\ensuremath{\Sigma_{#1}}\xspace}
\newcommand{\siw}[1]{\ensuremath{\Sigma_{#1}(<)}\xspace}
\newcommand{\siws}[1]{\ensuremath{\Sigma_{#1}(<,+1)}\xspace}
\newcommand{\siwm}[1]{\ensuremath{\Sigma_{#1}(<,\mods)}\xspace}
\newcommand{\siwam}[1]{\ensuremath{\Sigma_{#1}(<,\amods)}\xspace}
\newcommand{\siwsm}[1]{\ensuremath{\Sigma_{#1}(<,+1,\mods)}\xspace}
\newcommand{\siwsam}[1]{\ensuremath{\Sigma_{#1}(<,+1,\amods)}\xspace}
\newcommand{\siwss}[1]{\ensuremath{\Sigma_{#1}(<,+1,\min,\max,\varepsilon)}\xspace}
\newcommand{\siwssm}[1]{\ensuremath{\Sigma_{#1}(<,+1,\min,\max,\varepsilon,\mods)}\xspace}

\newcommand{\sici}{\sic{i}}
\newcommand{\siwi}{\siw{i}}
\newcommand{\siwsi}{\siws{i}}
\newcommand{\siwu}{\siw{1}}
\newcommand{\sicu}{\sic{1}}
\newcommand{\siwsu}{\siws{1}}
\newcommand{\sicd}{\sic{2}}
\newcommand{\siwd}{\siw{2}}
\newcommand{\siwsd}{\siws{2}}
\newcommand{\sict}{\sic{3}}
\newcommand{\siwt}{\siw{3}}
\newcommand{\siwst}{\siws{3}}
\newcommand{\sicq}{\sic{4}}
\newcommand{\siwq}{\siw{4}}
\newcommand{\siwsq}{\siws{4}}

% Pi
\newcommand{\pic}[1]{\ensuremath{\Pi_{#1}}\xspace}
\newcommand{\piw}[1]{\ensuremath{\Pi_{#1}(<)}\xspace}
\newcommand{\piws}[1]{\ensuremath{\Pi_{#1}(<,+1)}\xspace}
\newcommand{\piwm}[1]{\ensuremath{\Pi_{#1}(<,\mods)}\xspace}
\newcommand{\piwam}[1]{\ensuremath{\Pi_{#1}(<,\amods)}\xspace}
\newcommand{\piwsm}[1]{\ensuremath{\Pi_{#1}(<,+1,\mods)}\xspace}
\newcommand{\piwsam}[1]{\ensuremath{\Pi_{#1}(<,+1,\amods)}\xspace}
\newcommand{\piwss}[1]{\ensuremath{\Pi_{#1}(<,+1,\min,\max,\varepsilon)}\xspace}


\newcommand{\pici}{\pic{i}}
\newcommand{\piwi}{\piw{i}}
\newcommand{\piwsi}{\piws{i}}
\newcommand{\piwu}{\piw{1}}
\newcommand{\picu}{\pic{1}}
\newcommand{\piwsu}{\piws{1}}
\newcommand{\picd}{\pic{2}}
\newcommand{\piwd}{\piw{2}}
\newcommand{\piwsd}{\piws{2}}
\newcommand{\pict}{\pic{3}}
\newcommand{\piwt}{\piw{3}}
\newcommand{\piwst}{\piws{3}}
\newcommand{\picq}{\pic{4}}
\newcommand{\piwq}{\piw{4}}
\newcommand{\piwsq}{\piws{4}}

% Delta
\newcommand{\dec}[1]{\ensuremath{\Delta_{#1}}\xspace}
\newcommand{\dew}[1]{\ensuremath{\Delta_{#1}(<)}\xspace}
\newcommand{\dews}[1]{\ensuremath{\Delta_{#1}(<,+1)}\xspace}
\newcommand{\dewm}[1]{\ensuremath{\Delta_{#1}(<,\mods)}\xspace}
\newcommand{\dewam}[1]{\ensuremath{\Delta_{#1}(<,\amods)}\xspace}
\newcommand{\dewsm}[1]{\ensuremath{\Delta_{#1}(<,+1,\mods)}\xspace}
\newcommand{\dewsam}[1]{\ensuremath{\Delta_{#1}(<,+1,\amods)}\xspace}
\newcommand{\dewss}[1]{\ensuremath{\Delta_{#1}(<,+1,\min,\max,\varepsilon)}\xspace}

\newcommand{\deci}{\dec{i}}
\newcommand{\dewi}{\dew{i}}
\newcommand{\dewsi}{\dews{i}}
\newcommand{\dewu}{\dew{1}}
\newcommand{\decu}{\dec{1}}
\newcommand{\dewsu}{\dews{1}}
\newcommand{\decd}{\dec{2}}
\newcommand{\dewd}{\dew{2}}
\newcommand{\dewsd}{\dews{2}}
\newcommand{\dewmd}{\dewm{2}}
\newcommand{\dewamd}{\dewam{2}}
\newcommand{\dewsmd}{\dewsm{2}}
\newcommand{\dewsamd}{\dewsam{2}}
\newcommand{\dect}{\dec{3}}
\newcommand{\dewt}{\dew{3}}
\newcommand{\dewst}{\dews{3}}
\newcommand{\decq}{\dec{4}}
\newcommand{\dewq}{\dew{4}}
\newcommand{\dewsq}{\dews{4}}

% BSigma
\newcommand{\bsc}[1]{\ensuremath{\Bs\Sigma_{#1}}\xspace}
\newcommand{\bsw}[1]{\ensuremath{\Bs\Sigma_{#1}(<)}\xspace}
\newcommand{\bswm}[1]{\ensuremath{\Bs\Sigma_{#1}(<,\mods)}\xspace}
\newcommand{\bswam}[1]{\ensuremath{\Bs\Sigma_{#1}(<,\amods)}\xspace}
\newcommand{\bsws}[1]{\ensuremath{\Bs\Sigma_{#1}(<,+1)}\xspace}
\newcommand{\bswsm}[1]{\ensuremath{\Bs\Sigma_{#1}(<,+1,\mods)}\xspace}
\newcommand{\bswsam}[1]{\ensuremath{\Bs\Sigma_{#1}(<,+1,\amods)}\xspace}
\newcommand{\bswss}[1]{\ensuremath{\Bs\Sigma_{#1}(<,+1,\min,\max,\varepsilon)}\xspace}

\newcommand{\bsci}{\bsc{i}}
\newcommand{\bswi}{\bsw{i}}
\newcommand{\bswsi}{\bsws{i}}
\newcommand{\bswu}{\bsw{1}}
\newcommand{\bscu}{\bsc{1}}
\newcommand{\bswsu}{\bsws{1}}
\newcommand{\bscd}{\bsc{2}}
\newcommand{\bswd}{\bsw{2}}
\newcommand{\bswsd}{\bsws{2}}
\newcommand{\bsct}{\bsc{3}}
\newcommand{\bswt}{\bsw{3}}
\newcommand{\bswst}{\bsws{3}}
\newcommand{\bscq}{\bsc{4}}
\newcommand{\bswq}{\bsw{4}}
\newcommand{\bswsq}{\bsws{4}}


%%%%%%%%%%%% Regular Expressions %%%%%%%%%%%%%%

\newcommand{\ppt}{\ensuremath{\textup{PPT}}\xspace}
\newcommand{\pptp}[1]{\ensuremath{#1\textup{-}\textup{PPT}}\xspace}
\newcommand{\kppt}{\pptp{k}}
\newcommand{\pt}{\ensuremath{\textup{PT}}\xspace}
\newcommand{\ptp}[1]{\ensuremath{#1\textup{-}\textup{PT}}\xspace}
\newcommand{\kpt}{\ptp{k}}
\renewcommand{\ul}{\ensuremath{\textup{UL}}\xspace}
\newcommand{\ld}{\ensuremath{\textup{LD}}\xspace}
\newcommand{\rd}{\ensuremath{\textup{RD}}\xspace}


%%%%%%%%%%%% Language Theoritic %%%%%%%%%%%%%%
\newcommand{\wat}{\ensuremath{\textup{WAT}}\xspace}
\newcommand{\at}{\ensuremath{\textup{AT}}\xspace}

\newcommand{\cgrp}{\ensuremath{\textup{Ab}}\xspace}
\newcommand{\grp}{\ensuremath{\textup{GR}}\xspace}
\newcommand{\sgrp}{\ensuremath{\textup{SGR}}\xspace}

\newcommand{\abg}{\ensuremath{\textup{AMT}}\xspace}
\newcommand{\sabg}{\ensuremath{\textup{SAMT}}\xspace}
\newcommand{\pabg}[1]{\ensuremath{#1\textup{-}\textup{AMT}}\xspace}
\newcommand{\dabg}{\pabg{d}}

\newcommand{\md}{\ensuremath{\textup{MOD}}\xspace}
\newcommand{\smd}{\ensuremath{\textup{SMOD}}\xspace}
\newcommand{\pmd}[1]{\ensuremath{#1\textup{-}\textup{MOD}}\xspace}
\newcommand{\dmd}{\pmd{d}}


\newcommand{\pr}{\ensuremath{\textup{PR}}\xspace}
\newcommand{\wpr}{\ensuremath{\textup{PPR}}\xspace}
\newcommand{\prp}[1]{\ensuremath{#1\textup{-}\textup{PR}}\xspace}
\newcommand{\kpr}{\prp{k}}

\newcommand{\wsu}{\ensuremath{\textup{PSU}}\xspace}
\newcommand{\su}{\ensuremath{\textup{SU}}\xspace}
\newcommand{\psu}[1]{\ensuremath{#1\textup{-}\textup{SU}}\xspace}
\newcommand{\ksu}{\psu{k}}

\newcommand{\sfr}{\ensuremath{\textup{SF}}\xspace}
\newcommand{\sfrp}[1]{\ensuremath{#1\textup{-}\textup{SF}}\xspace}
\newcommand{\ksfr}{\sfrp{k}}
\newcommand{\bsd}{\ensuremath{\textup{SD}}\xspace}

\newcommand{\patt}[1]{\ensuremath{\ensuremath{#1\textup{-ATT}}}\xspace}
\newcommand{\datt}{\patt{d}}
\newcommand{\att}{\ensuremath{\textup{ATT}}\xspace}

\newcommand{\plt}[1]{\ensuremath{#1\textup{-LT}}\xspace}
\newcommand{\pltt}[2]{\ensuremath{(#1,#2)\textup{-LTT}}\xspace}
\newcommand{\klt}{\plt{k}}
\newcommand{\kdltt}{\pltt{k}{d}}
\newcommand{\lt}{\ensuremath{\textup{LT}}\xspace}
\newcommand{\ltt}{\ensuremath{\textup{LTT}}\xspace}
\newcommand{\lmt}{\ensuremath{\textup{LMT}}\xspace}

\newcommand{\stzer}{\textup{ST}\xspace}
\newcommand{\dotzer}{\textup{DD}\xspace}

\newcommand{\sttp}[1]{\hiep{\stzer}{#1}}
\newcommand{\dotdp}[1]{\hiep{\dotzer}{#1}}
\newcommand{\mdp}[1]{\hiep{\md}{#1}}
\newcommand{\abgp}[1]{\hiep{\abg}{#1}}
\newcommand{\grpp}[1]{\hiep{\grp}{#1}}
\newcommand{\mdwp}[1]{\hiep{\smd}{#1}}
\newcommand{\abgwp}[1]{\hiep{\sabg}{#1}}
\newcommand{\grpwp}[1]{\hiep{\sgrp}{#1}}



\newcommand{\sthone}{\sttp{{1}/{2}}}
\newcommand{\stone}{\sttp{1}}
\newcommand{\sthtwo}{\sttp{{3}/{2}}}
\newcommand{\sttwo}{\sttp{2}}
\newcommand{\sththree}{\sttp{{5}/{2}}}
\newcommand{\stthree}{\sttp{3}}
\newcommand{\sthfour}{\sttp{{7}/{2}}}
\newcommand{\stfour}{\sttp{4}}


\newcommand{\dothone}{\dotdp{{1}/{2}}}
\newcommand{\dotone}{\dotdp{1}}
\newcommand{\dothtwo}{\dotdp{{3}/{2}}}
\newcommand{\dottwo}{\dotdp{2}}
\newcommand{\doththree}{\dotdp{{5}/{2}}}
\newcommand{\dotthree}{\dotdp{3}}
\newcommand{\dothfour}{\dotdp{{7}/{2}}}
\newcommand{\dotfour}{\dotdp{4}}



%%%%%%%%%%%% Closure Operations %%%%%%%%%%%%%%

\newcommand{\cocl}[1]{\ensuremath{\mathit{co\textup{-}}\!#1}\xspace}
\newcommand{\bool}[1]{\ensuremath{\textup{Bool}(#1)}\xspace}
\newcommand{\pol}[1]{\ensuremath{\textup{Pol}(#1)}\xspace}
\newcommand{\bpol}[1]{\ensuremath{\textup{BPol}(#1)}\xspace}
\newcommand{\pbpol}[1]{\ensuremath{\textup{PBPol}(#1)}\xspace}
\newcommand{\upol}[1]{\ensuremath{\textup{UPol}(#1)}\xspace}
\newcommand{\spol}[1]{\ensuremath{\textup{SPol}(#1)}\xspace}
\newcommand{\copol}[1]{\ensuremath{\cocl{\textup{Pol}(#1)}}\xspace}
\newcommand{\capol}[1]{\ensuremath{\pol{#1} \cap \copol{#1}}\xspace}
\newcommand{\sfp}[1]{\ensuremath{\textup{\textup{SF}}(#1)}\xspace}
\newcommand{\bsdp}[1]{\ensuremath{\textup{\textup{SD}}(#1)}\xspace}
\newcommand{\dsdp}[1]{\ensuremath{\textup{\textup{DSD}}(#1)}\xspace}
\newcommand{\upolo}{\ensuremath{\textup{UPol}}\xspace}
\newcommand{\bpolo}{\ensuremath{\textup{BPol}}\xspace}
\newcommand{\polo}{\ensuremath{\textup{Pol}}\xspace}
\newcommand{\boolo}{\ensuremath{\textup{Bool}}\xspace}

% Generic operator
\newcommand{\opo}{\ensuremath{\textup{Op}}\xspace}

\newcommand{\booln}{\ensuremath{\textup{Bool}}\xspace}
\newcommand{\poln}{\ensuremath{\textup{Pol}}\xspace}
\newcommand{\bpoln}{\ensuremath{\textup{BPol}}\xspace}
\newcommand{\pbpoln}{\ensuremath{\textup{PBPol}}\xspace}
\newcommand{\sfpn}{\ensuremath{\textup{SF}}\xspace}

\newcommand{\ldet}[1]{\ensuremath{\textup{LPol}(#1)}\xspace}
\newcommand{\rdet}[1]{\ensuremath{\textup{RPol}(#1)}\xspace}
\newcommand{\adet}[1]{\ensuremath{\textup{APol}(#1)}\xspace}
\newcommand{\wadet}[1]{\ensuremath{\textup{WAPol}(#1)}\xspace}

\newcommand{\idet}[1]{\ensuremath{\ldet{#1} \cap \rdet{#1}}\xspace}
\newcommand{\jdet}[1]{\ensuremath{\ldet{#1} \vee \rdet{#1}}\xspace}
\newcommand{\mdet}[1]{\ensuremath{\textup{MPol}(#1)}\xspace}
\newcommand{\ldeto}{\ensuremath{\textup{LPol}}\xspace}
\newcommand{\rdeto}{\ensuremath{\textup{RPol}}\xspace}
\newcommand{\adeto}{\ensuremath{\textup{APol}}\xspace}
\newcommand{\wadeto}{\ensuremath{\textup{WAPol}}\xspace}
\newcommand{\ideto}{\ensuremath{\textup{IPol}}\xspace}
\newcommand{\jdeto}{\ensuremath{\textup{JPol}}\xspace}
\newcommand{\mdeto}{\ensuremath{\textup{MPol}}\xspace}

\newcommand{\ldetp}[2]{\ensuremath{\ldeto_{#1}(#2)}\xspace}
\newcommand{\rdetp}[2]{\ensuremath{\rdeto_{#1}(#2)}\xspace}
\newcommand{\mdetp}[2]{\ensuremath{\mdeto_{#1}(#2)}\xspace}
\newcommand{\idetp}[2]{\ensuremath{\ldetp{#1}{#2} \cap \rdetp{#1}{#2}}\xspace}
\newcommand{\jdetp}[2]{\ensuremath{\ldetp{#1}{#2} \vee \rdetp{#1}{#2}}\xspace}
\newcommand{\ldetn}[1]{\ldetp{n}{#1}}
\newcommand{\rdetn}[1]{\rdetp{n}{#1}}
\newcommand{\mdetn}[1]{\mdetp{n}{#1}}
\newcommand{\idetn}[1]{\idetp{n}{#1}}
\newcommand{\jdetn}[1]{\jdetp{n}{#1}}

\newcommand{\polp}[2]{\ensuremath{Pol_{#2}(#1)}\xspace}
\newcommand{\polk}[1]{\polp{#1}{k}}

\newcommand{\bpolp}[2]{\ensuremath{BPol_{#2}(#1)}\xspace}
\newcommand{\bpolk}[1]{\bpolp{#1}{k}}


%%%%%%%%%%%% Algebraic varieties %%%%%%%%%%%%%%
\newcommand{\meda}{\ensuremath{\textup{\sffamily M}_e\textup{\sffamily DA}}\xspace}
\newcommand{\davar}{\ensuremath{\textup{\sffamily DA}}\xspace}
\newcommand{\ldavar}{\ensuremath{\mathbf{LDA}}\xspace}
\newcommand{\jvar}{\ensuremath{\mathbf{J}}\xspace}

%%%%%%%%%%%% Temporal Logic %%%%%%%%%%%%%%



\newcommand{\tls}{\ensuremath{\textup{TL}}\xspace}
\newcommand{\tlxs}{\ensuremath{\textup{TLX}}\xspace}
\newcommand{\tla}[1]{\ensuremath{\tls[#1]}\xspace}
\newcommand{\tlxa}[1]{\ensuremath{\tlxs[#1]}\xspace}
\newcommand{\tlc}[1]{\ensuremath{\tls(#1)}\xspace}
\newcommand{\tlxc}[1]{\ensuremath{\tlxs(#1)}\xspace}

\newcommand{\tlsn}[1]{\ensuremath{\textup{TL}_{#1}}\xspace}
\newcommand{\tlxsn}[1]{\ensuremath{\textup{TLX}_{#1}}\xspace}
\newcommand{\tlna}[2]{\ensuremath{\tlsn{#1}[#2]}\xspace}
\newcommand{\tlxna}[2]{\ensuremath{\tlxsn{#1}[#2]}\xspace}
\newcommand{\tlnc}[2]{\ensuremath{\tlsn{#1}(#2)}\xspace}
\newcommand{\tlxnc}[2]{\ensuremath{\tlxsn{#1}(#2)}\xspace}

\newcommand{\btlsn}[1]{\ensuremath{\Bs\textup{TL}_{#1}}\xspace}
\newcommand{\btlxsn}[1]{\ensuremath{\Bs\textup{TLX}_{#1}}\xspace}
\newcommand{\btlna}[2]{\ensuremath{\btlsn{#1}[#2]}\xspace}
\newcommand{\btlxna}[2]{\ensuremath{\btlxsn{#1}[#2]}\xspace}
\newcommand{\btlnc}[2]{\ensuremath{\btlsn{#1}(#2)}\xspace}
\newcommand{\btlxnc}[2]{\ensuremath{\btlxsn{#1}(#2)}\xspace}




\newcommand{\tlb}[1]{\ensuremath{\textup{BL}^{#1}}\xspace}
\newcommand{\tlf}[1]{\ensuremath{\textup{FL}^{#1}}\xspace}
\newcommand{\tlp}[1]{\ensuremath{\textup{PL}^{#1}}\xspace}

\newcommand{\tlfo}{\ensuremath{\textup{FL}}\xspace}
\newcommand{\tlpo}{\ensuremath{\textup{PL}}\xspace}

\newcommand{\tlxb}[1]{\ensuremath{\textup{BLX}^{#1}}\xspace}
\newcommand{\tlxf}[1]{\ensuremath{\textup{FLX}^{#1}}\xspace}
\newcommand{\tlxp}[1]{\ensuremath{\textup{PLX}^{#1}}\xspace}

\newcommand{\tlbc}[2]{\ensuremath{\tlb{#1}(#2)}\xspace}
\newcommand{\tlfc}[2]{\ensuremath{\tlf{#1}(#2)}\xspace}
\newcommand{\tlpc}[2]{\ensuremath{\tlp{#1}(#2)}\xspace}

\newcommand{\tlfoc}[1]{\ensuremath{\tlfo(#1)}\xspace}
\newcommand{\tlpoc}[1]{\ensuremath{\tlpo(#1)}\xspace}


\newcommand{\tlba}[2]{\ensuremath{\tlb{#1}[#2]}\xspace}
\newcommand{\tlfa}[2]{\ensuremath{\tlf{#1}[#2]}\xspace}
\newcommand{\tlpa}[2]{\ensuremath{\tlp{#1}[#2]}\xspace}

\newcommand{\tlfoa}[1]{\ensuremath{\tlfo[#1]}\xspace}
\newcommand{\tlpoa}[1]{\ensuremath{\tlpo[#1]}\xspace}

\newcommand{\tlxbc}[2]{\ensuremath{\tlxb{#1}(#2)}\xspace}
\newcommand{\tlxfc}[2]{\ensuremath{\tlxf{#1}(#2)}\xspace}
\newcommand{\tlxpc}[2]{\ensuremath{\tlxp{#1}(#2)}\xspace}

\newcommand{\tlxba}[2]{\ensuremath{\tlxb{#1}[#2]}\xspace}
\newcommand{\tlxfa}[2]{\ensuremath{\tlxf{#1}[#2]}\xspace}
\newcommand{\tlxpa}[2]{\ensuremath{\tlxp{#1}[#2]}\xspace}

\newcommand{\ltl}{\ensuremath{\textup{LTL}}\xspace}
\newcommand{\ltlp}{\ensuremath{\textup{LTLP}}\xspace}


\newcommand{\ltla}[1]{\ensuremath{\ltl[#1]}\xspace}
\newcommand{\ltlpa}[1]{\ensuremath{\ltlp[#1]}\xspace}

\newcommand{\ltlc}[1]{\ensuremath{\ltl(#1)}\xspace}
\newcommand{\ltlpc}[1]{\ensuremath{\ltlp(#1)}\xspace}

%%%%%%%%%% Temporal Logic Operators %%%%%%%%%


\newcommand{\until}[2]{\ensuremath{#1~\textup{U}~#2}\xspace}
\newcommand{\finally}[1]{\mbox{\ensuremath{\textup{F}\,#1}}\xspace}
\newcommand{\nex}[1]{{\ensuremath{\textup{X}\,#1}}\xspace}
\newcommand{\since}[2]{\ensuremath{#1~\textup{S}~#2}\xspace}
\newcommand{\finallym}[1]{\ensuremath{\textup{P}~#1}\xspace}
\newcommand{\nexm}[1]{\ensuremath{\textup{Y}~#1}\xspace}




\newcommand{\untilp}[3]{\ensuremath{#2~\textup{U}_{#1}~#3}\xspace}
\newcommand{\sincep}[3]{\ensuremath{#2~\textup{S}_{#1}~#3}\xspace}

\newcommand{\finallyi}[2]{\ensuremath{\textup{F}^{#2}~#1}\xspace}
\newcommand{\finallymi}[2]{\ensuremath{\textup{P}^{#2}~#1}\xspace}
\newcommand{\nexi}[2]{\ensuremath{\textup{X}^{#2}~#1}\xspace}
\newcommand{\nexmi}[2]{\ensuremath{\textup{Y}^{#2}~#1}\xspace}

\newcommand{\finallyp}[2]{\mbox{\ensuremath{\textup{F}_{#1}\,#2}}\xspace}
\newcommand{\finallymp}[2]{\ensuremath{\textup{P}_{#1}\,#2}\xspace}
\newcommand{\finallyl}[1]{\finallyp{L}{#1}}
\newcommand{\finallyml}[1]{\finallymp{L}{#1}}

\newcommand{\xfinallyp}[2]{\ensuremath{\textup{F}^{sa}_{#1}\,#2}\xspace}
\newcommand{\xfinallymp}[2]{\ensuremath{\textup{P}^{sa}_{#1}\,#2}\xspace}


%%%%%%%%%% Determinsitic constructions %%%%%%


\newcommand{\clp}[2]{\ensuremath{[#1]_{#2}}\xspace}
\newcommand{\cle}[1]{\clp{#1}{\eta}}
\newcommand{\clg}[1]{\clp{#1}{\gamma}}
\newcommand{\cla}[1]{\clp{#1}{\alpha}}
\newcommand{\clz}[1]{\clp{#1}{\zeta}}

\newcommand{\eqlp}[1]{\ensuremath{\mathrel{\rhd_{#1}}}\xspace}
\newcommand{\eqlaep}[1]{\eqlp{\alpha,\eta,#1}}
\newcommand{\eqlaek}{\eqlaep{k}}
\newcommand{\eqlep}[1]{\eqlp{\eta,#1}}
\newcommand{\eqlek}{\eqlep{k}}
\newcommand{\eqrp}[1]{\ensuremath{\mathrel{\lhd_{#1}}}\xspace}
\newcommand{\eqraep}[1]{\eqrp{\alpha,\eta,#1}}
\newcommand{\eqraek}{\eqraep{k}}
\newcommand{\eqrep}[1]{\eqrp{\eta,#1}}
\newcommand{\eqrek}{\eqrep{k}}
\newcommand{\eqmp}[1]{\ensuremath{\mathrel{\bowtie_{#1}}}\xspace}
\newcommand{\eqmaep}[1]{\eqmp{\alpha,\eta,#1}}
\newcommand{\eqmaek}{\eqmaep{k}}
\newcommand{\eqmep}[1]{\eqmp{\eta,#1}}
\newcommand{\eqmek}{\eqmep{k}}
\newcommand{\eqmap}[1]{\eqmp{\alpha,#1}}
\newcommand{\eqmak}{\eqmap{k}}

\newcommand{\cllp}[2]{\ensuremath{[#1]_{\rhd,#2}}\xspace}
\newcommand{\cllaep}[2]{\cllp{#1}{\alpha,\eta,#2}}
\newcommand{\cllaek}[1]{\cllaep{#1}{k}}
\newcommand{\cllep}[2]{\cllp{#1}{\eta,#2}}
\newcommand{\cllek}[1]{\cllep{#1}{k}}
\newcommand{\clrp}[2]{\ensuremath{[#1]_{\lhd,#2}}\xspace}
\newcommand{\clraep}[2]{\clrp{#1}{\alpha,\eta,#2}}
\newcommand{\clraek}[1]{\clraep{#1}{k}}
\newcommand{\clrep}[2]{\clrp{#1}{\eta,#2}}
\newcommand{\clrek}[1]{\clrep{#1}{k}}
\newcommand{\clmp}[2]{\ensuremath{[#1]_{\bowtie,#2}}\xspace}
\newcommand{\clmaep}[2]{\clmp{#1}{\alpha,\eta,#2}}
\newcommand{\clmaek}[1]{\clmaep{#1}{k}}
\newcommand{\clmep}[2]{\clmp{#1}{\eta,#2}}
\newcommand{\clmek}[1]{\clmep{#1}{k}}


\newcommand{\poslp}[3]{\ensuremath{\poschar_{\triangleright}(#1,#2,#3)}\xspace}
\newcommand{\posrp}[3]{\ensuremath{\poschar_{\triangleleft}(#1,#2,#3)}\xspace}
\newcommand{\posmp}[3]{\ensuremath{\poschar_{\bowtie}(#1,#2,#3)}\xspace}
\newcommand{\posup}[3]{\ensuremath{\poschar_{\infty}(#1,#2,#3)}\xspace}
\newcommand{\poslak}[1]{\poslp{\alpha}{k}{#1}}
\newcommand{\posrak}[1]{\posrp{\alpha}{k}{#1}}
\newcommand{\posmak}[1]{\posmp{\alpha}{k}{#1}}
\newcommand{\poslek}[1]{\poslp{\eta}{k}{#1}}
\newcommand{\posrek}[1]{\posrp{\eta}{k}{#1}}
\newcommand{\posmek}[1]{\posmp{\eta}{k}{#1}}
\newcommand{\posuek}[1]{\posup{\eta}{k}{#1}}


%%%%% Equ temporal %%%%

\newcommand{\tleqp}[1]{\ensuremath{\cong_{\eta,#1}}\xspace}
\newcommand{\tleqk}{\tleqp{k}}
\newcommand{\tldp}[1]{\ensuremath{\cong_{\delta,#1}}\xspace}
\newcommand{\tldk}{\tldp{k}}

\newcommand{\qtlp}[1]{\ensuremath{\preceq_{\eta,#1}}\xspace}
\newcommand{\qtlkn}{\qtlp{k,n}}
\newcommand{\eqtlp}[1]{\ensuremath{\cong_{\eta,#1}}\xspace}
\newcommand{\eqtlkn}{\eqtlp{k,n}}
\newcommand{\qtldp}[1]{\ensuremath{\preceq_{\delta,#1}}\xspace}
\newcommand{\qtldkn}{\qtldp{k,n}}

%\textup{F} \textup{P}

\newcommand{\tlfeqp}[1]{\ensuremath{\blacktriangleright_{\eta,#1}}\xspace}
\newcommand{\tlfeqk}{\tlfeqp{k}}
\newcommand{\tlfdqp}[1]{\ensuremath{\blacktriangleright_{\delta,#1}}\xspace}
\newcommand{\tlfdqk}{\tlfdqp{k}}

\newcommand{\tlpeqp}[2]{\ensuremath{\blacktriangleleft_{#1,\eta,#2}}\xspace}
\newcommand{\tlpeqkn}{\tlpeqp{n}{k}}
\newcommand{\tlpdp}[2]{\ensuremath{\blacktriangleleft_{#1,\delta,#2}}\xspace}
\newcommand{\tlpdkn}{\tlpdp{n}{k}}


%%%%%

\newcommand{\lbi}{\ensuremath{f_{\triangleright}}\xspace}
\newcommand{\rbi}{\ensuremath{f_{\triangleleft}}\xspace}


%%%% Green

\newcommand{\Jrel}{\ensuremath{\mathrel{\mathscr{J}}}\xspace}
\newcommand{\Hrel}{\ensuremath{\mathrel{\mathscr{H}}}\xspace}
\newcommand{\Rrel}{\ensuremath{\mathrel{\mathscr{R}}}\xspace}
\newcommand{\Lrel}{\ensuremath{\mathrel{\mathscr{L}}}\xspace}
\newcommand{\Drel}{\ensuremath{\mathrel{\mathscr{D}}}\xspace}

\newcommand{\Jord}{\ensuremath{\leqslant_{\mathscr{J}}}\xspace}
\newcommand{\Hord}{\ensuremath{\leqslant_{\mathscr{H}}}\xspace}
\newcommand{\Rord}{\ensuremath{\leqslant_{\mathscr{R}}}\xspace}
\newcommand{\Lord}{\ensuremath{\leqslant_{\mathscr{L}}}\xspace}
\newcommand{\Dord}{\ensuremath{\leqslant_{\mathscr{D}}}\xspace}


\newcommand{\Jords}{\ensuremath{<_{\mathscr{J}}}\xspace}
\newcommand{\Hords}{\ensuremath{<_{\mathscr{H}}}\xspace}
\newcommand{\Rords}{\ensuremath{<_{\mathscr{R}}}\xspace}
\newcommand{\Lords}{\ensuremath{<_{\mathscr{L}}}\xspace}
\newcommand{\Dords}{\ensuremath{<_{\mathscr{D}}}\xspace}


%%% Pos

\newcommand{\poschar}{\textup{\sffamily{Pos}}}

\newcommand{\pos}[1]{\ensuremath{\poschar(#1)\xspace}}
\newcommand{\posc}[1]{\ensuremath{\poschar_{c}(#1)\xspace}}
\newcommand{\posl}[1]{\ensuremath{\poschar_{\ell}(#1)\xspace}}
\newcommand{\posr}[1]{\ensuremath{\poschar_{r}(#1)\xspace}}

\newcommand{\infix}[3]{\ensuremath{#1(#2,#3)}\xspace}
\newcommand{\suffix}[2]{\infix{#1}{#2}{|#1|+1}}
\newcommand{\prefix}[2]{\infix{#1}{0}{#2}}
\newcommand{\wpos}[2]{\ensuremath{#1[#2]}\xspace}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

